Vision Foundation Models in Remote Sensing: A Survey

Artificial Intelligence (AI) technologies have profoundly transformed the field of remote sensing, revolutionizing data collection, processing, and analysis. Traditionally reliant on manual interpretation and task-specific models, remote sensing research has been significantly enhanced by the advent of foundation models-large-scale, pre-trained AI models capable of performing a wide array of tasks with unprecedented accuracy and efficiency. This paper provides a comprehensive survey of foundation models in the remote sensing domain. We categorize these models based on their architectures, pre-training datasets, and methodologies. Through detailed performance comparisons, we highlight emerging trends and the significant advancements achieved by those foundation models. Additionally, we discuss technical challenges, practical implications, and future research directions, addressing the need for high-quality data, computational resources, and improved model generalization. Our research also finds that pre-training methods, particularly self-supervised learning techniques like contrastive learning and masked autoencoders, remarkably enhance the performance and robustness of foundation models. This survey aims to serve as a resource for researchers and practitioners by providing a panorama of advances and promising pathways for continued development and application of foundation models in remote sensing.

==> tables/CV_domain_backup.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table*}[]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{|cc|
>{\columncolor[HTML]{F3F3F3}}c c
>{\columncolor[HTML]{F3F3F3}}c c|
>{\columncolor[HTML]{F3F3F3}}l |}
\hline
\multicolumn{2}{|c|}{\cellcolor[HTML]{C9DAF8}} &
  \multicolumn{4}{c|}{\cellcolor[HTML]{C9DAF8}
    \parbox[c][1.15cm]{\linewidth}{\centering\textbf{\large Compute Vision Tasks}}} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{C9DAF8}} \\ \cline{3-6}
\multicolumn{2}{|c|}{\multirow{-2}{*}{\cellcolor[HTML]{C9DAF8}\centering\textbf{\Large Domain-Specific Tasks}}} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{CFE2F3}
    \parbox[c][4cm]{0.22\linewidth}{\centering\textbf{Classification} \\[0.1cm] \includegraphics[width=\linewidth]{pic_added/classification_wo_bg.png}}} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{CFE2F3}
    \parbox[c][4cm]{0.21\linewidth}{\centering\textbf{Segmentation\textsuperscript{*}} \\ \includegraphics[width=\linewidth]{pic_added/segmentation.png}}} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{CFE2F3}
      \parbox[c][4cm]{0.223\linewidth}{\centering\textbf{Object Detection\textsuperscript{*}} \\ \includegraphics[width=\linewidth]{pic_added/object_detection.png}}} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{CFE2F3}
      \parbox[c][4cm]{0.25\linewidth}{\centering\textbf{Spatial-Temporal \cite{Daudt2018}} \\ \includegraphics[width=\linewidth]{pic_added/spacial_tamporal.png}}} &
  \multicolumn{1}{c|}{\multirow{-2}{*}{\cellcolor[HTML]{C9DAF8}\centering\textbf{\Large Related Work}}} \\ \hline

% Environmental Monitoring \cellcolor[HTML]{F4CCCC}
\multicolumn{1}{|c|}{\multirow{8}{*}{
    \parbox[t][9cm]{0.6\linewidth}{\centering\textbf{\large Environmental Monitoring} \\[0.05cm] \includegraphics[width=\linewidth]{pic_added/environment.png}}}} &
    
\cellcolor[HTML]{F4CCCC} \begin{tabular}[c]{@{}c@{}}Land Cover \\ Change Detection\end{tabular} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{F3F3F3}} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{\parbox[c][1.1cm]{0.25\linewidth}{\centering \cellcolor[HTML]{F3F3F3}}} &
  \multicolumn{1}{c|}{\scalebox{2.5}{\centering$\checkmark$}} &
  \begin{tabular}[c]{@{}l@{}}\cite{SeCo, MATTER, RSP, RingMo, CMID, CACo, GFM, RingMo-lite, SwiMDiff, SpectralGPT} \\ \cite{SkySense, UPetu, DINO-MC, MTP, SoftCon, LeMeViT, S2MAE, A2-MAE, HyperSIGMA} \end{tabular} \\ \cline{2-7}
\multicolumn{1}{|c|}{} &
\cellcolor[HTML]{F4CCCC} \begin{tabular}[c]{@{}c@{}}Deforestation Monitoring \end{tabular} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{F3F3F3}} &
  \multicolumn{1}{c|}{\scalebox{2.5}{$\checkmark$}} &
  \multicolumn{1}{c|}{\parbox[c][1.2cm]{0.25\linewidth}{\centering \cellcolor[HTML]{F3F3F3}}} &
  \multicolumn{1}{c|}{} &
  \begin{tabular}[c]{@{}l@{}}
  \cite{GeoKR, MATTER, GASSL, RSP, Scheibenreif_2022_CVPR, RingMo, GeCo, RS-BYOL, RVSA, SatMAE,TOV} \\ 
  \cite{CMID, CACo, GFM, SatlasPretrain, RingMo-Sense, Scale-MAE, RingMo-lite, DeCUR, Feng2023} \\ 
  \cite{FG-MAE, CROMA, Cross-Scale-MAE, U-BARN, GeRSP, SMLFR, SpectralGPT, Presto, SkySense, UPetu} \\ 
  \cite{msGFM, OFA-Net, MTP, CtxMIM, SoftCon, LeMeViT, RS-DFM, A2-MAE, HyperSIGMA, DOFA} \end{tabular} \\ \cline{2-7}
  
\multicolumn{1}{|c|}{} &
\cellcolor[HTML]{F4CCCC}  \begin{tabular}[c]{@{}c@{}}Water Body Analysis \end{tabular} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{F3F3F3}} &
  \multicolumn{1}{c|}{\scalebox{2.5}{$\checkmark$}} &
  \multicolumn{1}{c|}{\parbox[c][1.2cm]{0.25\linewidth}{\centering \cellcolor[HTML]{F3F3F3}}\scalebox{2.5}{$\checkmark$}} & 
   \scalebox{2.5}{$\checkmark$}&
  \begin{tabular}[c|]{@{}l@{}} \cite{RSP, RingMo, CMID, Feng2023, SkySense, MTP, LeMeViT, HyperSIGMA}\end{tabular} \\ \cline{2-7} 

\multicolumn{1}{|c|}{} &
\cellcolor[HTML]{F4CCCC}  \begin{tabular}[c]{@{}c@{}}Forest \\ Cover mapping\end{tabular} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{F3F3F3}} &
  \multicolumn{1}{c|}{\scalebox{2.5}{$\checkmark$}} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{F3F3F3}} &
   \scalebox{2.5}{$\checkmark$}&
  \begin{tabular}[c|]{@{}l@{}}\cite{RSP, RingMo, CACo, GFM, RingMo-lite, Feng2023, SpectralGPT, SoftCon, LeMeViT}\\ \cite{S2MAE, A2-MAE, HyperSIGMA} \end{tabular}\\ \cline{2-7}
  
\multicolumn{1}{|c|}{} &
\cellcolor[HTML]{F4CCCC}  \begin{tabular}[c]{@{}c@{}}Biomass Estimation\end{tabular} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{F3F3F3}} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{\parbox[c][0.8cm]{0.25\linewidth}{\centering \cellcolor[HTML]{F3F3F3}}} &
  \scalebox{2.5}{} &
  \cite{IaI-SimCLR} \\ \cline{2-7}
\multicolumn{1}{|c|}{} &
\cellcolor[HTML]{F4CCCC}  \begin{tabular}[c]{@{}c@{}}Weather/Climate \\ Prediction \end{tabular} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{F3F3F3}\scalebox{2.5}{$\checkmark$}} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{\parbox[c][1cm]{0.25\linewidth}{\centering \cellcolor[HTML]{F3F3F3}}} &
   &
  \cite{EarthPT, RingMo-Sense, ORBIT} \\ \cline{2-7}
\multicolumn{1}{|c|}{} &
\cellcolor[HTML]{F4CCCC}  \begin{tabular}[c]{@{}c@{}}Cloud Removal\end{tabular} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{F3F3F3}} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{\parbox[c][0.9cm]{0.25\linewidth}{\centering \cellcolor[HTML]{F3F3F3}}} &
   &
  \cite{msGFM} \\ \cline{2-7}
\multicolumn{1}{|c|}{} &
\cellcolor[HTML]{F4CCCC}  \begin{tabular}[c]{@{}c@{}}Moisture Content \\ Measurement\end{tabular} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{F3F3F3}} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{\parbox[c][0.9cm]{0.25\linewidth}{\centering \cellcolor[HTML]{F3F3F3}}} &
   &
  \cite{Presto} \\ \hline


% Agriculture \cellcolor[HTML]{FCE5CD}
\multicolumn{1}{|c|}{\multirow{7}{*}{
    \parbox[t][10cm]{0.6\linewidth}{\centering\textbf{\large Agriculture} \\ \includegraphics[width=\linewidth]{pic_added/agriculture.png}}}} &
    
\cellcolor[HTML]{FCE5CD}  \begin{tabular}[c]{@{}c@{}}Crop Type Mapping\end{tabular} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{F3F3F3}\scalebox{2.5}{$\checkmark$}} &
  \multicolumn{1}{c|}{\scalebox{2.5}{$\checkmark$}} &
  \multicolumn{1}{c|}{\parbox[c][1.2cm]{0.25\linewidth}{\centering \cellcolor[HTML]{F3F3F3}\scalebox{2.5}{$\checkmark$}}} &
  \multicolumn{1}{c|}{\scalebox{2.5}{$\checkmark$}}&
  \cite{RSP, RingMo, CMID, Feng2023, SkySense, MTP, LeMeViT, HyperSIGMA, SSL4EO-L} \\ \cline{2-7}
\multicolumn{1}{|c|}{} &
\cellcolor[HTML]{FCE5CD}  \begin{tabular}[c]{@{}c@{}}Weed Detection\end{tabular} &
   \multicolumn{1}{c|}{\cellcolor[HTML]{F3F3F3}} &
   \multicolumn{1}{c|}{} &
   \multicolumn{1}{c|}{\parbox[c][1.2cm]{0.25\linewidth}{\centering \cellcolor[HTML]{F3F3F3}\scalebox{2.5}{$\checkmark$}}} & 
   &
  \begin{tabular}[c]{@{}l@{}}\cite{GeoKR, GASSL, RSP, RingMo, GeCo, CSPT, RVSA, TOV, CMID, Feng2023} \\ 
  \cite{FoMo-Bench, SkySense, MTP, CtxMIM, LeMeViT, RS-DFM, HyperSIGMA, SMLFR}\end{tabular} \\ \cline{2-7}
  
\multicolumn{1}{|c|}{} &
\cellcolor[HTML]{FCE5CD}  \begin{tabular}[c]{@{}c@{}}Disease  Monitoring\end{tabular} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{F3F3F3}\scalebox{2.5}{$\checkmark$}} &
  \multicolumn{1}{c|}{\parbox[c][1.2cm]{0.25\linewidth}{\centering \scalebox{2.5}{$\checkmark$}}} & 
  \multicolumn{1}{c|}{\cellcolor[HTML]{F3F3F3}} &
  \scalebox{2.5}{$\checkmark$} &
  \begin{tabular}[c]{@{}l@{}}
  \cite{GeoKR, GASSL, RSP, RingMo, GeCo, RVSA, TOV, CMID, Feng2023} \\ 
  \cite{SkySense, MTP, CtxMIM, LeMeViT, RS-DFM, HyperSIGMA, SMLFR} \end{tabular} \\ \cline{2-7}
\multicolumn{1}{|c|}{} &
\cellcolor[HTML]{FCE5CD} Forecasting &
  \multicolumn{1}{c|}{\parbox[c][1.2cm]{0.25\linewidth}{\centering \cellcolor[HTML]{F3F3F3}}} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{F3F3F3}} &
   &
  \cite{EarthPT, RingMo-Sense} \\ \cline{2-7}
\multicolumn{1}{|c|}{} &
\cellcolor[HTML]{FCE5CD}  \begin{tabular}[c]{@{}c@{}}Soil Parameter Estimation\end{tabular} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{F3F3F3}} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{\parbox[c][1.2cm]{0.25\linewidth}{\centering \cellcolor[HTML]{F3F3F3}}} &
   &
  \cite{DOFA} \\ \cline{2-7}
\multicolumn{1}{|c|}{} &
\cellcolor[HTML]{FCE5CD}  \begin{tabular}[c]{@{}c@{}}Yield  Estimation \end{tabular} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{F3F3F3}\scalebox{2.5}{$\checkmark$}} &
  \multicolumn{1}{c|}{\scalebox{2.5}{$\checkmark$}} &
  \multicolumn{1}{c|}{\parbox[c][1.2cm]{0.25\linewidth}{\centering \cellcolor[HTML]{F3F3F3}}} &
   &
  \begin{tabular}[c]{@{}l@{}}
  \cite{GeoKR, MATTER, GASSL, RSP, Scheibenreif_2022_CVPR, RingMo, GeCo, RS-BYOL, RVSA, SatMAE, TOV} \\ 
  \cite{CMID, CACo, GFM, SatlasPretrain, Scale-MAE, RingMo-lite, DeCUR, Feng2023} \\
  \cite{FG-MAE, Cross-Scale-MAE, U-BARN, GeRSP, SpectralGPT, SkySense, UPetu, msGFM, OFA-Net} \\
  \cite{MTP, CtxMIM, SoftCon, A2-MAE, HyperSIGMA, DOFA} \\ \end{tabular} \\ \cline{2-7} 
  
\multicolumn{1}{|c|}{} &
\cellcolor[HTML]{FCE5CD}  \begin{tabular}[c]{@{}c@{}}Agricultural Pattern \\ Segmentation\end{tabular} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{F3F3F3}} &
   \multicolumn{1}{c|}{\parbox[c][1.8cm]{0.25\linewidth}{\centering \scalebox{2.5}{$\checkmark$}}} & 

  \multicolumn{1}{c|}{\cellcolor[HTML]{F3F3F3}} &
   &
  \cite{SeCo} \\ \hline
  
% Archaeology \cellcolor[HTML]{FFF2CC}
\multicolumn{1}{|c|}{\multirow{5}{*}{
    \parbox[c][10cm][t]{0.6\linewidth}{\centering\textbf{\large Archaeology} \\[0.05cm] \includegraphics[width=\linewidth]{pic_added/archaeology_backup.png}}}} &

\cellcolor[HTML]{FFF2CC}\begin{tabular}[c]{@{}c@{}}Artifact Classification \\ and Recognition\end{tabular} &
 \multicolumn{1}{c|}{\parbox[c][1.45cm]{0.25\linewidth}{\centering \cellcolor[HTML]{F3F3F3}\scalebox{2.5}{$\checkmark$}}} & 
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{F3F3F3}\scalebox{2.5}{$\checkmark$}} &
   &
  \begin{tabular}[c]{@{}l@{}}
  \cite{CMC-RSSR, SeCo, GeoKR, MATTER, GASSL, RSP, DINO-MM, Scheibenreif_2022_CVPR, RingMo} \\
  \cite{CSPT, RVSA, SatMAE, TOV, CMID, CACo, IaI-SimCLR, GFM, SatlasPretrain, Scale-MAE, RingMo-lite} \\
  \cite{Feng2023, FG-MAE, USat, Cross-Scale-MAE, U-BARN, EarthPT, GeRSP, SwiMDiff, SAR-JEPA} \\
  \cite{FoMo-Bench, SkySense, UPetu, msGFM, DINO-MC, OFA-Net, MTP, MMEarth, CtxMIM, SoftCon} \\
  \cite{RS-BYOL, GeCo, DOFA,  HyperSIGMA, DeCUR, SpectralGPT, S2MAE,A2-MAE}\end{tabular} \\ \cline{2-7}
  
\multicolumn{1}{|c|}{} &
\cellcolor[HTML]{FFF2CC}  \begin{tabular}[c]{@{}c@{}}Detection of \\ Archaeological Structures\end{tabular} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{F3F3F3}} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{\parbox[c][2cm]{0.25\linewidth}{\centering \cellcolor[HTML]{F3F3F3}\scalebox{2.5}{$\checkmark$}}} & 
   &
  \begin{tabular}[c]{@{}l@{}}\cite{GeoKR, GASSL, RSP, RingMo, GeCo, CSPT, RVSA, TOV, CMID, Feng2023} \\ 
  \cite{FoMo-Bench, SkySense, MTP, CtxMIM, LeMeViT, RS-DFM, HyperSIGMA, SMLFR}\end{tabular} \\ \cline{2-7}
\multicolumn{1}{|c|}{} &
\cellcolor[HTML]{FFF2CC}  \begin{tabular}[c]{@{}c@{}}Semantic \\ Segmentation\end{tabular} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{F3F3F3}} &
  \multicolumn{1}{c|}{\parbox[c][2cm]{0.25\linewidth}{\centering \scalebox{2.5}{$\checkmark$}}} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{F3F3F3}} &
   &
  \begin{tabular}[c]{@{}l@{}}
  \cite{GeoKR, MATTER, GASSL, RSP, Scheibenreif_2022_CVPR, RingMo, GeCo, RS-BYOL, RVSA, SatMAE,TOV} \\ 
  \cite{CMID, CACo, GFM, SatlasPretrain, RingMo-Sense, Scale-MAE, RingMo-lite, DeCUR, Feng2023} \\ 
  \cite{FG-MAE, CROMA, Cross-Scale-MAE, U-BARN, GeRSP, SMLFR, SpectralGPT, Presto, SkySense, UPetu} \\ 
  \cite{msGFM, OFA-Net, MTP, CtxMIM, SoftCon, LeMeViT, RS-DFM, A2-MAE, HyperSIGMA, DOFA} \end{tabular} \\ \cline{2-7}
\multicolumn{1}{|c|}{} &
\cellcolor[HTML]{FFF2CC}  \begin{tabular}[c]{@{}c@{}}Texture/Structural \\ Analysis\end{tabular} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{F3F3F3}} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{\parbox[c][2cm]{0.25\linewidth}{\centering \cellcolor[HTML]{F3F3F3}}} & 
   &
   \cite{MATTER} \\ \cline{2-7}
\multicolumn{1}{|c|}{} &
\cellcolor[HTML]{FFF2CC}  \begin{tabular}[c]{@{}c@{}}Pattern Recognition\end{tabular} &
  \multicolumn{1}{c|}{\parbox[c][1.6cm]{0.25\linewidth}{\centering \cellcolor[HTML]{F3F3F3}}} &
  \multicolumn{1}{c|}{\scalebox{2.5}{$\checkmark$}} &
  \multicolumn{1}{c|}{\parbox[c][1.6cm]{0.25\linewidth}{\centering \cellcolor[HTML]{F3F3F3}\scalebox{2.5}{$\checkmark$}}}& 
   &
   \begin{tabular}[c]{@{}l@{}}\cite{GeoKR, GASSL, RSP, RingMo, GeCo, RVSA, TOV, CMID, Feng2023} \\ \cite{SkySense, MTP, CtxMIM, LeMeViT, RS-DFM, HyperSIGMA, SMLFR} \end{tabular} \\ \hline

% Urban Planning and Development \cellcolor[HTML]{D9EAD3}
\multicolumn{1}{|c|}{\multirow{7}{*}{
    \parbox[t][7cm]{0.6\linewidth}{\centering\textbf{\large Urban Planning \& Development} \\[0.1cm] \includegraphics[width=\linewidth]{pic_added/urban.png}}}} &

\cellcolor[HTML]{D9EAD3}  \begin{tabular}[c]{@{}c@{}}Traffic Monitoring\end{tabular} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{F3F3F3}\scalebox{2.5}{$\checkmark$}} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{\parbox[c][1.5cm]{0.25\linewidth}{\centering \cellcolor[HTML]{F3F3F3}\scalebox{2.5}{$\checkmark$}}} &
  \scalebox{2.5}{$\checkmark$} &
  \cite{RSP, RingMo, CMID, Feng2023, SkySense, MTP, LeMeViT, HyperSIGMA} \\ \cline{2-7}
\multicolumn{1}{|c|}{} &
\cellcolor[HTML]{D9EAD3}  \begin{tabular}[c]{@{}c@{}}Land Cover/Use \\ Classification\end{tabular} &
  \multicolumn{1}{c|}{\parbox[c][1.8cm]{0.25\linewidth}{\centering \cellcolor[HTML]{F3F3F3}\scalebox{2.5}{$\checkmark$}}} & 
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{F3F3F3}} &
   &
  \begin{tabular}[c]{@{}l@{}}
  \cite{CMC-RSSR, SeCo, GeoKR, MATTER, GASSL, RSP, DINO-MM, Scheibenreif_2022_CVPR, RingMo} \\
  \cite{CSPT, RVSA, SatMAE, TOV, CMID, CACo, IaI-SimCLR, GFM, SatlasPretrain, Scale-MAE, RingMo-lite} \\
  \cite{Feng2023, FG-MAE, USat, Cross-Scale-MAE, U-BARN, EarthPT, GeRSP, SwiMDiff, SAR-JEPA} \\
  \cite{FoMo-Bench, SkySense, UPetu, msGFM, DINO-MC, OFA-Net, MTP, MMEarth, CtxMIM, SoftCon} \\
  \cite{RS-BYOL, GeCo, DOFA, HyperSIGMA, DeCUR, SpectralGPT, S2MAE,A2-MAE, SSL4EO-L}\end{tabular} \\ \cline{2-7}
\multicolumn{1}{|c|}{} &
\cellcolor[HTML]{D9EAD3}  \begin{tabular}[c]{@{}c@{}}Road Crack Detection\end{tabular} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{F3F3F3}} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{\parbox[c][1.2cm]{0.25\linewidth}{\centering \cellcolor[HTML]{F3F3F3}\scalebox{2.5}{$\checkmark$}}} &
   &
   \begin{tabular}[c]{@{}l@{}}\cite{GeoKR, GASSL, RSP, RingMo, GeCo, CSPT, RVSA, TOV, CMID, Feng2023} \\ 
  \cite{FoMo-Bench, SkySense, MTP, CtxMIM, LeMeViT, RS-DFM, HyperSIGMA, SMLFR}\end{tabular} \\ \cline{2-7}
\multicolumn{1}{|c|}{} &
\cellcolor[HTML]{D9EAD3}  \begin{tabular}[c]{@{}c@{}}Air Quality Monitoring\end{tabular} &
  \multicolumn{1}{c|}{\parbox[c][1.2cm]{0.25\linewidth}{\centering \cellcolor[HTML]{F3F3F3}\scalebox{2.5}{$\checkmark$}}}&
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{F3F3F3}\scalebox{2.5}{$\checkmark$}} &
   &
  \begin{tabular}[c]{@{}l@{}}\cite{msGFM, GeoKR, GASSL, RSP, RingMo, GeCo, RVSA, TOV, CMID,Feng2023} \\ \cite{SkySense, MTP, CtxMIM, LeMeViT, RS-DFM, HyperSIGMA, SMLFR} \end{tabular} \\ \cline{2-7}
\multicolumn{1}{|c|}{} &
\cellcolor[HTML]{D9EAD3}  \begin{tabular}[c]{@{}c@{}}Building Extraction\end{tabular} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{F3F3F3}\scalebox{2.5}{$\checkmark$}} &
  \multicolumn{1}{c|}{\parbox[c][1.2cm]{0.25\linewidth}{\centering \scalebox{2.5}{$\checkmark$}}} & 
  \multicolumn{1}{c|}{\cellcolor[HTML]{F3F3F3}} &
   &
  \cite{Feng2023} \\ \cline{2-7}
\multicolumn{1}{|c|}{} &
\cellcolor[HTML]{D9EAD3}  \begin{tabular}[c]{@{}c@{}}Object/Video Tracking\end{tabular} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{F3F3F3}} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{F3F3F3}\scalebox{2.5}{$\checkmark$}} &
  \scalebox{2.5}{$\checkmark$} &
  \cite{RingMo-Sense} \\ \cline{2-7}
\multicolumn{1}{|c|}{} &
\cellcolor[HTML]{D9EAD3}  \begin{tabular}[c]{@{}c@{}}Infrastructure \\ Monitoring\end{tabular} &
  \multicolumn{1}{c|}{\parbox[c][1.8cm]{0.25\linewidth}{\centering \cellcolor[HTML]{F3F3F3}}} & 
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{F3F3F3}} &
   &
  \cite{RingMo-Sense, USat} \\ \hline

% Disaster Management \cellcolor[HTML]{D9D2E9}
\multicolumn{1}{|c|}{\multirow{7}{*}{
    \parbox[t][4cm][t]{0.6\linewidth}{\centering\textbf{\large Disaster Management} \\\includegraphics[width=\linewidth]{pic_added/disaster.png}}}} &

\cellcolor[HTML]{D9D2E9}  \begin{tabular}[c]{@{}c@{}}Landslide Risk Monitoring\end{tabular} &
   \multicolumn{1}{c|}{\parbox[c][1.4cm]{0.25\linewidth}{\centering \cellcolor[HTML]{F3F3F3}}\scalebox{2.5}{$\checkmark$}} & 
  \multicolumn{1}{c|}{\scalebox{2.5}{$\checkmark$}} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{F3F3F3}\scalebox{2.5}{$\checkmark$}} &
  \scalebox{2.5}{$\checkmark$} &
  \cite{RSP, RingMo, CMID, Feng2023, SkySense, MTP, LeMeViT, HyperSIGMA} \\ \cline{2-7}
\multicolumn{1}{|c|}{} &
\cellcolor[HTML]{D9D2E9}  \begin{tabular}[c]{@{}c@{}}Disaster Response\end{tabular} &
  \multicolumn{1}{c|}{\parbox[c][0.9cm]{0.25\linewidth}{\centering \cellcolor[HTML]{F3F3F3}}} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{F3F3F3}} &
   &
   \cite{DOFA} \\ \cline{2-7}
\multicolumn{1}{|c|}{} &
\cellcolor[HTML]{D9D2E9}  \begin{tabular}[c]{@{}c@{}}Real-Time Detection \\ and Mapping\end{tabular} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{F3F3F3}} &
  \multicolumn{1}{c|}{\scalebox{2.5}{$\checkmark$}} &
  \multicolumn{1}{c|}{\parbox[c][1.2cm]{0.25\linewidth}{\centering \cellcolor[HTML]{F3F3F3}\scalebox{2.5}{$\checkmark$}}} &
  \scalebox{2.5}{$\checkmark$} &
  \cite{RSP, RingMo, CMID, Feng2023, SkySense, MTP, LeMeViT, HyperSIGMA} \\ \cline{2-7}
\multicolumn{1}{|c|}{} &
\cellcolor[HTML]{D9D2E9}  \begin{tabular}[c]{@{}c@{}}Building Damage \\ Assessment\end{tabular} &
  \multicolumn{1}{c|}{\parbox[c][1cm]{0.25\linewidth}{\centering \cellcolor[HTML]{F3F3F3}} \scalebox{2.5}{$\checkmark$}} &
  \multicolumn{1}{c|}{\scalebox{2.5}{$\checkmark$}} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{F3F3F3} \scalebox{2.5}{$\checkmark$}} &
   &
  \cite{RSP, RingMo, CMID, Feng2023, SkySense, MTP, LeMeViT, HyperSIGMA} \\ \cline{2-7}
\multicolumn{1}{|c|}{} &
\cellcolor[HTML]{D9D2E9}  \begin{tabular}[c]{@{}c@{}}Critical Infrastructure \\ Detection\end{tabular} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{F3F3F3}\scalebox{2.5}{$\checkmark$}} &
  \multicolumn{1}{c|}{} &
 \multicolumn{1}{c|}{\parbox[c][1.8cm]{0.25\linewidth}{\centering \cellcolor[HTML]{F3F3F3}\scalebox{2.5}{$\checkmark$}}} & 
 &
  \begin{tabular}[c]{@{}c@{}} \cite{GeoKR, GASSL, RSP, RingMo, GeCo, CSPT, RVSA, TOV, CMID, Feng2023} \\ 
  \cite{FoMo-Bench, SkySense, MTP, CtxMIM, LeMeViT, RS-DFM, HyperSIGMA, SMLFR}\end{tabular} \\ \cline{2-7}
\multicolumn{1}{|c|}{} &
\cellcolor[HTML]{D9D2E9}  \begin{tabular}[c]{@{}c@{}}Flood/Fire Mapping and Prediction\end{tabular} &
  \multicolumn{1}{c|}{\parbox[c][1.4cm]{0.25\linewidth}{\centering \cellcolor[HTML]{F3F3F3}\scalebox{2.5}{$\checkmark$}}} &
  \multicolumn{1}{c|}{\scalebox{2.5}{$\checkmark$}} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{F3F3F3}} &
  \scalebox{2.5}{$\checkmark$} &
  \begin{tabular}[c]{@{}c@{}} \cite{RSP, RingMo, CACo, GFM, RingMo-lite, Feng2023, SpectralGPT} \\ 
  \cite{SoftCon, LeMeViT, A2-MAE, HyperSIGMA}\end{tabular} \\ \cline{2-7}
\multicolumn{1}{|c|}{} &
\cellcolor[HTML]{D9D2E9}  \begin{tabular}[c]{@{}c@{}}Crowd and Vehicle Detection\end{tabular} &
  \multicolumn{1}{c|}{\parbox[c][1.4cm]{0.25\linewidth}{\centering \cellcolor[HTML]{F3F3F3}}} &
  \multicolumn{1}{c|}{} &
  \multicolumn{1}{c|}{\cellcolor[HTML]{F3F3F3}\scalebox{2.5}{$\checkmark$}} &
  \scalebox{2.5}{$\checkmark$} &
    \begin{tabular}[c]{@{}l@{}}\cite{SeCo, MATTER, RSP, RingMo, CMID, CACo, GFM, RingMo-lite, SwiMDiff, SpectralGPT} \\ \cite{SkySense, UPetu, DINO-MC, MTP, SoftCon, LeMeViT, S2MAE, A2-MAE, HyperSIGMA} \end{tabular} \\ \hline
\end{tabular}
}
\caption{This diagram illustrates various domain-specific tasks in computer vision and their connections. Key areas include Environmental Monitoring, Agriculture, Urban Planning and Development, Disaster Management, and Archaeology. Each domain comprises specific tasks such as classification, segmentation, change detection and object detection. The relationships between these tasks and their application domains are depicted through checkmarks, emphasizing the interconnected nature of computer vision applications across different fields. \\ \textsuperscript{*}© MAXAR 2024, provided through the NextView License Agreement.}
\end{table*}

\label{tab:cv-domain}



==> tables/Used_Scene_Classification.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}
\begin{sidewaystable*}[]
\centering
\begin{adjustbox}{width=\textwidth}{!}{%
\begin{tabular}{cc
>{\columncolor[HTML]{FFF2CC}}c cccccc} 
\cellcolor[HTML]{D9E7FD}\textbf{Year-Month} &
  \cellcolor[HTML]{D9E7FD}\textbf{Architecture} &
  \cellcolor[HTML]{D9EAD3}\textbf{Model Name} &
  \cellcolor[HTML]{D9E7FD}\textbf{Pre-training Dataset} &
  \cellcolor[HTML]{D9E7FD}\textbf{Resolution (m)} &
  \cellcolor[HTML]{D9E7FD}\textbf{Geographic Coverage} &
  \cellcolor[HTML]{D9E7FD}\textbf{Visual Encoder} &
  \cellcolor[HTML]{D9E7FD}\textbf{Pretrain Methods} &
  \cellcolor[HTML]{D9E7FD}\textbf{\# of Params} \\ 
2021 Oct &
  ResNet-50 &
  GeoKR \cite{GeoKR} &
  Levir-KR \cite{GeoKR}&
  0.8 to 16 &
  Global &
  ResNet-50/VGG16 &
  \begin{tabular}[c]{@{}c@{}}Geographical Knowledge\\ Supervision\end{tabular} &
  23.5M/138M \\
2021 Oct &
  ResNet-50 &
  SeCo \cite{SeCo}&
  Sentinel-2 Imagery &
  10, 20, and 60 &
  \begin{tabular}[c]{@{}c@{}}200k Locations \\ Worldwide\end{tabular} &
  ResNet-50 &
  CL &
  23.5M \\
2022 Jun &
  ViT-S/8 &
  DINO-MM \cite{DINO-MM}&
  BigEarthNet - MM &
  10 &
  Global &
  ViT-S/8 &
  SSL &
  22M \\
2023 Jan &
  \begin{tabular}[c]{@{}c@{}}MAE-based \\ Framework\end{tabular} &
  SatMAE \cite{SatMAE} &
  fMoW Sentinal-2 &
  10, 20, 60 &
  Global &
  ViT-Large &
  MAE &
  307M \\
2022 Sep &
  BYOL &
  RS-BYOL \cite{RS-BYOL}&
  Sen12MS \cite{schmitt2019sen12mscurateddataset}&
  10 to 20 &
  Global &
  ResNet-50 &
  SSL &
  23.5M \\
2022 Aug &
  ResNet-50 &
  GeCO \cite{GeCo}&
  Levir-KR \cite{GeoKR}&
  0.8 to 16 &
  Global &
  ResNet-50 &
  SSL &
  23.5M \\
2022 Jul &
  ViT/Swin Transformer &
  RingMo \cite{RingMo}&
  2 million RS images &
  0.3 to 30 &
  6 Continents &
  ViT/Swin Transformer &
  MIM &
  - \\
2022 Nov &
  ViT &
  RVSA \cite{RVSA}&
  MillionAID \cite{Long2022ASP_millionaid, Long2021DiRS_millionaid}&
  0.5 to 153 &
  Global &
  ViT-B/ViTAE-B &
  MAE &
  100M \\
2021 Dec &
  ResNet-34 &
  MATTER \cite{MATTER}&
  Sentinel-2 Imagery &
  - &
  \begin{tabular}[c]{@{}c@{}}Rural and Remote Regions\\ with Little Changes\end{tabular} &
  ResNet-34 &
  SSL &
  21.3M \\
2022 Nov &
  ViT-B &
  CSPT \cite{CSPT}&
  ImageNet-1K &
  - &
  Global &
  ViT-B &
  SSL &
  86M \\
2022 Jun &
  Swin Transformer &
  Scheibenreif, et al. \cite{Scheibenreif_2022_CVPR}&
  SEN12MS &
  10 &
  Global &
  Swim Transformer &
  CL &
  - \\
2023 Apr &
  TOV &
  TOV \cite{TOV}&
  \begin{tabular}[c]{@{}c@{}}TOV-NI,\\ TOV-RS\end{tabular} &
  - &
  Global &
  ViT &
  SSL &
  - \\
2023 Apr &
  \begin{tabular}[c]{@{}c@{}}Teacher-student\\ Self-distillation\end{tabular} &
  CMID \cite{CMID}&
  MillionAID \cite{Long2022ASP_millionaid, Long2021DiRS_millionaid}&
  Varied &
  Global &
  ResNet-50/Swin-B &
  SSL &
  25.6M/87.8M \\
2023 Jun &
  ResNet-18 &
  IaI-SimCLR \cite{IaI-SimCLR}&
  SEN12MS &
  - &
  Global &
  ResNet-18 &
  CL &
  11.7M \\
2023 Jun &
  CACo &
  CACo \cite{CACo}&
  Sentinel-2 Imagery &
  10 &
  Global &
  ResNet-18/50 &
  SSL &
  11.7M/23.5M \\
2023 Aug &
  Swim Transformer &
  SatLasPretrain \cite{SatlasPretrain} &
  SatLasPretrain &
  1, 10 &
  All Continents except Antarctica &
  Swim Transformer &
  Pretrained on Dataset &
  88M \\   % changed based on 
2023 Aug &
  Teacher-Student &
  GFM \cite{GFM}&
  GeoPile &
  - &
  Global &
  Swim Transformer &
  Continual Pretraining &
  - \\
2023 Sep &
  ViT &
  Scale-MAE \cite{Scale-MAE}&
  FMoW \cite{fmow2018}&
  - &
  Global &
  ViT-Large &
  MAE &
  322.9M \\
2024 Apr &
  DINO &
  DINO-MC \cite{DINO-MC}&
  SeCo-100K \cite{SeCo}&
  10 to 60 &
  Global &
  \begin{tabular}[c]{@{}c@{}}ViT,\\ Swim Transformer,\\ ResNet,\\ WRN\end{tabular} &
  SSL &
  - \\
2023 Nov &
  Multimodal Encoder &
  CROMA \cite{CROMA}&
  SSL4EO \cite{wang2023ssl4eos12largescalemultimodalmultitemporal}&
  10 &
  \begin{tabular}[c]{@{}c@{}}Areas Surrounding \\ Human Settlements\end{tabular} &
  ViT-B &
  CL, MAE &
  86M \\
2024 Jan &
  ViT-B &
  Cross-Scale MAE \cite{Cross-Scale-MAE}&
  fMoW \cite{fmow2018}&
  - &
  Global &
  ViT-B &
  MAE &
  86M \\
2023 Sep &
  Multimodel SSL &
  DeCUR \cite{DeCUR}&
  \begin{tabular}[c]{@{}c@{}}SSL4EO-S12, \\ RGB-DEM/depth\end{tabular} &
  Varied &
  Global &
  ResNet-50 &
  SSL &
  23.5M \\
2024 May &
  ViT &
  CtxMIM \cite{CtxMIM}&
  WorldView-3 Imagery &
  Varied &
  Asia &
  Swim-B &
  MIM &
  88M \\
2023 Oct &
  ViT &
  FG-MAE \cite{FG-MAE}&
  SSL4EO-S12 \cite{wang2023ssl4eos12largescalemultimodalmultitemporal}&
  10 &
  Global &
  ViT &
  MAE &
  - \\
2023 Sep &
  CNN-Transformer &
  RingMo-lite \cite{RingMo-lite}&
  AID \cite{Xia_2017}&
  0.3 to 30 &
  Global &
  Swim Transformer + CNN &
  FD-MIM &
  60\% less than RingMo \\
2023 Oct &
  MSFE+MMFH &
  Feng et al. \cite{Feng2023}&
  Multi-modal Dataset &
  Varied &
  Global &
  Transformer &
  SSL &
  - \\
2024 Jan &
  ViT &
  USat \cite{USat}&
  Satlas &
  Varied &
  Global &
  ViT &
  MAE &
  - \\
2024 Mar &
  ViT &
  FoMo-Bench \cite{FoMo-Bench}&
  Multiple &
  Varied &
  Global &
  ViT &
  MAE &
  101M/110M \\
2024 Jan &
  Unet+Transformer &
  U-BARN \cite{U-BARN}&
  Sentinel-2 Imagery &
  Varied &
  France &
  Unet+Transformer &
  SSL &
  - \\
2024 Jan &
  \begin{tabular}[c]{@{}c@{}}Teacher-Student \\ Network\end{tabular} &
  GeRSP \cite{GeRSP}&
  ImageNet\cite{imageNet}, MillionAID\cite{Long2022ASP_millionaid, Long2021DiRS_millionaid} &
  0.5 to 153 &
  Global &
  ResNet-50 &
  SSL, SL &
  - \\
2024 Jan &
  Dual-Branch &
  SwiMDiff \cite{SwiMDiff}&
  Sen12MS \cite{schmitt2019sen12mscurateddataset} &
  Varied &
  Global &
  ResNet-18 &
  SSL &
  11.7M \\
2024 May &
  OFA-Net &
  OFA-Net \cite{OFA-Net}&
  Multi-modal Dataset &
  Varied &
  Global &
  ViT &
  MIM &
  - \\
2024 Feb &
  3D GPT &
  SpectralGPT \cite{SpectralGPT}&
  Sentinel-2 Imagery &
  Varied &
  Global &
  ViT &
  MAE &
  100M/300M/600M \\
2024 May &
  HiViT &
  SARATR-X \cite{SARATR-X}&
  SAR Datasets &
  0.1 to 3 &
  Global &
  HiViT &
  MIM &
  66M \\
2024 Mar &
  SatMAE &
  SatMAE++ \cite{SatMAE++}&
  fMoW \cite{fmow2018} &
  Varied &
  Global &
  ViT-Large &
  \begin{tabular}[c]{@{}c@{}}Multi-Scale\\ Pre-training\end{tabular} &
  - \\
2024 Apr &
  Swim Transformer &
  msGFM \cite{msGFM}&
  GeoPile-2 &
  0.1 to 153 &
  Global &
  Swim Transformer &
  MIM &
  89M \\
2024 Mar &
  \begin{tabular}[c]{@{}c@{}}Factorized Multi-Modal\\ Spatiotemporal Encoder\end{tabular} &
  SkySense \cite{SkySense}&
  Multiple &
  Varied &
  Global &
  Multiple &
  CL &
  2.06B \\
2024 May &
  \begin{tabular}[c]{@{}c@{}}Shared Encoder\\ Task-Specific Decoders\end{tabular} &
  MTP \cite{MTP}&
  SAMRS &
  Varied &
  Global &
  \begin{tabular}[c]{@{}c@{}}RVSA,\\ InternImage\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Multi-Task \\ Pretraining\end{tabular} &
  over 300M \\
2024 Jun &
  Dynamic OFA &
  DOFA \cite{DOFA}&
  Multiple &
  Varied &
  Global &
  ViT &
  MIM &
  - \\
2024 Mar &
  Multi-Modules &
  UPetu \cite{UPetu}&
  GeoSense &
  - &
  Global &
  ConvNeXt-B &
  SSL &
  0.65M \\
2024 May &
  MP-MAE &
  MMEarth \cite{MMEarth}&
  \begin{tabular}[c]{@{}c@{}}Multi-modal,\\ Geospatial Data\end{tabular} &
  - &
  Global &
  ConvNeXt V2 &
  MP-MAE &
  3.7M to 650M
\end{tabular}%
}
\end{adjustbox}
\caption{Summary of foundation models for scene classification in remote sensing, detailing architecture, pre-training datasets, resolution, geographic coverage, visual encoders, pretraining methods, and number of parameters.}
\label{tab:scene_classification}
\end{sidewaystable*}

==> tables/Used_change_detection.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}
\begin{sidewaystable*}
\centering
\begin{adjustbox}{width=\textwidth}{!}{%
\begin{tabular}{cc
>{\columncolor[HTML]{FFF2CC}}c cccccc}
\cellcolor[HTML]{D9E7FD}\textbf{Year-Month} &
  \cellcolor[HTML]{D9E7FD}\textbf{Architecture} &
  \cellcolor[HTML]{D9EAD3}\textbf{Model Name} &
  \cellcolor[HTML]{D9E7FD}\textbf{Pre-training Dataset} &
  \cellcolor[HTML]{D9E7FD}\textbf{Resolution (m)} &
  \cellcolor[HTML]{D9E7FD}\textbf{Geographic Coverage} &
  \cellcolor[HTML]{D9E7FD}\textbf{Visual encoder} &
  \cellcolor[HTML]{D9E7FD}\textbf{Pretrain methods} &
  \cellcolor[HTML]{D9E7FD}\textbf{\# of Params} \\
2021 Oct &
  ResNet-50 &
  SeCo\cite{SeCo} &
  Sentinel-2 imagery &
  10, 20, 60 &
  200k Locations Worldwide &
  ResNet-50 &
  CL &
  23.5M \\
2022 Jul &
  ViT/Swin Transformer &
  RingMo\cite{RingMo} &
  2M RS images &
  0.3 to 30 &
  6 Continents &
  ViT/Swin Transformer &
  MIM &
  - \\
2022 May &
  ViT &
  RSP\cite{RSP} &
  MillionAID &
  0.5 to 153 &
  Global &
  ViTAEv2-S/ ResNet-50/Swin-T &
  Supervised Learning &
  24.8M/23.5M/29M \\
2021 Dec &
  ResNet-34 &
  MATTER\cite{MATTER} &
  Sentinel-2 imagery &
  - &
  \begin{tabular}[c]{@{}c@{}}Rural and Remote Regions \\with Little Change \end{tabular}&
  ResNet34 &
  SSL &
  21.3M \\
2023 Apr &
  \begin{tabular}[c]{@{}c@{}}Teacher-Student\\     Self-distillation\end{tabular}&
  CMID\cite{CMID} &
  MillionAID &
  Varied &
  Global &
  ResNet-50/Swin-B &
  SSL &
  25.6M/87.8M \\
2023 Jun &
  CACo &
  CACo\cite{CACo} &
  Sentinel-2 imagery &
  10 &
  Global &
  ResNet-18/50 &
  SSL &
  11.7M/23.5M \\
2023 Aug &
  Teacher-Student &
  GFM\cite{GFM} &
  GeoPile &
  - &
  Global &
  Swim Transformer &
  Continual Pretraining &
  - \\
2024 Apr &
  DINO &
  DINO-MC\cite{DINO-MC} &
  SeCo-100K &
  10 to 60 &
  Global &
  \begin{tabular}[c]{@{}c@{}}ViT,\\      Swim Transformer,\\      ResNet,\\      WRN\end{tabular} &
  SSL &
  - \\
2023 Sep &
  CNN-Transformer &
  RingMo-lite\cite{RingMo-lite} &
  AID &
  0.3 to 30 &
  Global &
  Swim Transformer, CNN &
  FD-MIM &
  60\% less than RingMo \\
2023 Oct &
  MSFE+MMFH &
  Feng et al.\cite{Feng2023}&
   Multi-modal Dataset &
  Varied &
  Global &
  Transformer &
  SSL &
  - \\
2024 Jan &
  Dual-Branch &
  SwiMDiff\cite{SwiMDiff} &
  Sen12MS &
  Varied &
  Global &
  ResNet-18 &
  SSL &
  11.7M \\
2024 Feb &
  3D GPT &
  SpectralGPT\cite{SpectralGPT} &
  Sentinel-2 Imagery &
  Varied &
  Global &
  ViT &
  MAE &
  100M/300M/600M \\
2024 Mar &
  \begin{tabular}[c]{@{}c@{}}Factorized Multi-Modal\\Spatiotemporal Encoder\end{tabular}   &
  SkySense\cite{SkySense} &
  Multiple &
  Varied &
  Global &
  Multiple &
  CL &
  2.06B \\
2024 May &
  \begin{tabular}[c]{@{}c@{}}Shared Encoder+\\Task-Specific Decoders\end{tabular} &
  MTP\cite{MTP} &
  SAMRS &
  Varied &
  Global &
  RVSA, InternImage &
  Multi-Task Learning &
  over 300M
\end{tabular}%
}
\end{adjustbox}
\caption{Summary of foundation models for change detection in remote sensing, detailing architecture, pre-training datasets, resolution, geographic coverage, visual encoders, pretraining methods, and number of parameters.}
\label{tab:change_detection}
\end{sidewaystable*}

==> tables/Used_object_detection.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}

\begin{sidewaystable*}
\centering
\begin{adjustbox}{width=\textwidth}{!}{%
\begin{tabular}{cc
>{\columncolor[HTML]{FFF2CC}}c cccccc}
\cellcolor[HTML]{D9E7FD}\textbf{Year-Month} &
  \cellcolor[HTML]{D9E7FD}\textbf{Architecture} &
  \cellcolor[HTML]{D9EAD3}\textbf{Model Name} &
  \cellcolor[HTML]{D9E7FD}\textbf{Pre-training Dataset} &
  \cellcolor[HTML]{D9E7FD}\textbf{Resolution (m)} &
  \cellcolor[HTML]{D9E7FD}\textbf{Geographic Coverage} &
  \cellcolor[HTML]{D9E7FD}\textbf{visual encoder (backbone)} &
  \cellcolor[HTML]{D9E7FD}\textbf{Pretrain methods} &
  \cellcolor[HTML]{D9E7FD}\textbf{\# of Params} \\
2021 Oct &
  ResNet-50 &
  GeoKR \cite{GeoKR} &
  Levir-KR \cite{GeoKR} &
  0.8 to 16 &
  Global &
  ResNet-50/VGG16 &
  \begin{tabular}[c]{@{}c@{}}Geographical Knowledge\\ Supervision\end{tabular} &
  23.5M/138M \\
2021 Oct &
  ResNet-50 &
  SeCo \cite{SeCo}&
  Sentinel-2 Imagery &
  10, 20, 60 &
  \begin{tabular}[c]{@{}c@{}}200k Locations \\ Worldwide\end{tabular} &
  ResNet-50 &
  CL &
  23.5M \\
2022 Aug &
  ResNet-50 &
  GeCO \cite{GeCo}&
  Levir-KR \cite{GeoKR}&
  0.8 to 16 &
  Global &
  ResNet-50 &
  SSL &
  23.5M \\
2022 Jul &
  ViT/Swin Transformer &
  RingMo \cite{RingMo}&
  2 Million RS Images &
  0.3 to 30 &
  6 Continents &
  ViT/Swin Transformer &
  MIM &
  - \\
2022 Nov &
  ViT &
  RVSA \cite{RVSA}&
  MillionAID \cite{Long2022ASP_millionaid, Long2021DiRS_millionaid}&
  0.5 to 153 &
  Global &
  ViT-B/ViTAE-B &
  MAE &
  100M \\
2022 May &
  ViTAEv2-S &
  RSP \cite{RSP}&
  MillionAID \cite{Long2022ASP_millionaid, Long2021DiRS_millionaid} &
  0.5 to 153 &
  Global &
  ViTAEv2-S/ ResNet-50/Swin-T &
  Supervised Learning &
  24.8M/23.5M/29M \\
2022 Nov &
  ViT-B &
  CSPT \cite{CSPT}&
  ImageNet-1K &
  - &
  Global &
  ViT-B &
  SSL &
  86M \\
2024 May &
  ViT &
  BFM \cite{BFM}&
  MillionAID \cite{Long2022ASP_millionaid, Long2021DiRS_millionaid}&
  0.5 to 153 &
  Global &
  ViT &
  MAE &
  86M/605.26M/1.36B/2.42B \\
2023 Apr &
  TOV &
  TOV \cite{TOV}&
  \begin{tabular}[c]{@{}c@{}}TOV-NI,\\ TOV-RS\end{tabular} &
  - &
  Global &
  ViT &
  SSL &
  - \\
2023 Apr &
  \begin{tabular}[c]{@{}c@{}}Teacher-student\\ Self-distillation\end{tabular} &
  CMID \cite{CMID}&
  MillionAID \cite{Long2022ASP_millionaid, Long2021DiRS_millionaid} &
  Varied &
  Global &
  ResNet-50/Swin-B &
  SSL &
  25.6M/87.8M \\
2023 Sep &
  Multi-Branch &
  RingMo-Sense \cite{RingMo-Sense}&
  \begin{tabular}[c]{@{}c@{}}RS Spatiotemporal \\ Dataset\end{tabular} &
  - &
  Global &
  Video Swim Transformer &
  SSL &
  - \\
2024 Feb &
  \begin{tabular}[c]{@{}c@{}}MAE-based \\ Framework\end{tabular} &
  Presto \cite{Presto}&
  Presto-21.5M &
  10 &
  Global &
  Transformer-based &
  MAE &
  402K \\
2024 May &
  ViT &
  CtxMIM \cite{CtxMIM}&
  \begin{tabular}[c]{@{}c@{}}WorldView-3 \\ Imagery\end{tabular} &
  Varied &
  Asia &
  Swim-B &
  MIM &
  88M \\
2023 Sep &
  CNN-Transformer &
  RingMo-lite \cite{RingMo-lite}&
  AID \cite{Xia_2017} &
  0.3 to 30 &
  Global &
  Swim Transformer + CNN &
  FD-MIM &
  60\% less than RingMo \\
2023 Oct &
  MSFE+MMFH &
  Feng et al. \cite{Feng2023}&
  \begin{tabular}[c]{@{}c@{}}Multi-modal \\ Dataset\end{tabular} &
  Varied &
  Global &
  Transformer &
  SSL &
  - \\
2024 Jan &
  ViT &
  USat \cite{USat}&
  Satlas &
  Varied &
  Global &
  ViT &
  MAE &
  - \\
2024 March &
  ViT &
  FoMo-Bench \cite{FoMo-Bench}&
  Multiple &
  Varied &
  Global &
  ViT &
  MAE &
  101M/110M \\
2024 Jan &
  \begin{tabular}[c]{@{}c@{}}Teacher-Student \\ Network\end{tabular} &
  GeRSP \cite{GeRSP}&
  \begin{tabular}[c]{@{}c@{}}ImageNet, \\ MillionAID \cite{Long2022ASP_millionaid, Long2021DiRS_millionaid}\end{tabular} &
  0.5 to 153 &
  Global &
  ResNet-50 &
  SSL, SL &
  - \\
2024 Jan &
  Generative ConvNet &
  SMLFR \cite{SMLFR}&
  GeoSense &
  0.05 to 150 &
  Multiple Continents &
  ConvNeXt &
  SSL &
  88M/197M \\
2024 May &
  HiViT &
  SARATR-X \cite{SARATR-X}&
  SAR Datasets &
  0.1 to 3 &
  Global &
  HiViT &
  MIM &
  66M \\
2024 Mar &
  \begin{tabular}[c]{@{}c@{}}Factorized Multi-Modal\\ Spatiotemporal Encoder\end{tabular} &
  SkySense \cite{SkySense}&
  Multiple &
  Varied &
  Global &
  Multiple &
  CL &
  2.06B \\
2024 May &
  \begin{tabular}[c]{@{}c@{}}Shared Encoder+\\ Task-Specific Decoders\end{tabular} &
  MTP \cite{MTP}&
  SAMRS &
  Varied &
  Global &
  RVSA, InternImage &
  Multi-Task Pretraining &
  over 300M \\
2024 Jun &
  Dynamic OFA &
  DOFA \cite{DOFA}&
  Multiple &
  Varied &
  Global &
  ViT &
  MIM &
  -
\end{tabular}%
}
\end{adjustbox}
\caption{Summary of foundation models for object detection in remote sensing, detailing architecture, pre-training datasets, resolution, geographic coverage, visual encoders, pretraining methods, and number of parameters.}
\label{tab:object_detection}
\end{sidewaystable*}


==> tables/Used_pre-train_datasets.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{sidewaystable*}
\centering
\begin{adjustbox}{width=\textwidth}{!}{%
\begin{tabular}{c|
>{\columncolor[HTML]{DAE8FC}}c |ccccccccc}
\cellcolor[HTML]{FFCCC9}\textbf{Month, Year} &
  \cellcolor[HTML]{FFCC67}\textbf{Dataset} &
  \cellcolor[HTML]{FFCCC9}\textbf{Title} &
  \cellcolor[HTML]{FFCCC9}\textbf{Patch Size} &
  \cellcolor[HTML]{FFCCC9}\textbf{Size} &
  \cellcolor[HTML]{FFCCC9}\textbf{Resolution (m)} &
  \cellcolor[HTML]{FFCCC9}\textbf{Source} &
  \cellcolor[HTML]{FFCCC9}\textbf{Categories} &
  \cellcolor[HTML]{FFCCC9}\textbf{Geographic Coverage} &
  \cellcolor[HTML]{FFCCC9}\textbf{Image Type} &
  \cellcolor[HTML]{FFCCC9}\textbf{Application} \\ \hline
2017 &
  RSD46-WHU \cite{Long2017, Xiao2017} &
  - &
  256 x 256 &
  117,000 &
  0.5 - 2 &
  \begin{tabular}[c]{@{}c@{}}Google Earth, \\ Tianditu\end{tabular} &
  46 &
  Global &
  RGB &
  Scene Classification \\
Apr, 2018 &
  fMoW \cite{fmow2018} &
  Functional Map of the World &
  - &
  1,047,691 &
  - &
  Digital Globe &
  63 &
  207 of 247 countries &
  Multispectral &
  \begin{tabular}[c]{@{}c@{}}Scene Classification, \\ Object Detection\end{tabular} \\
May, 2019 &
  DOTA \cite{xia2019dotalargescaledatasetobject} &
  \begin{tabular}[c]{@{}c@{}}DOTA: A Large-scale Dataset for Object \\ Detection in Aerial Images\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}800 × 800 \\ to 20,000 × 20,000\end{tabular} &
  11,268 &
  Various &
  \begin{tabular}[c]{@{}c@{}}Google Earth, \\ GF-2 Satellite, \\ and aerial images\end{tabular} &
  18 &
  Global &
  RGB &
  Object Detection \\
Jun, 2019 &
  SEN12MS \cite{schmitt2019sen12mscurateddataset} &
  \begin{tabular}[c]{@{}c@{}}SEN12MS -- A Curated Dataset of \\ Georeferenced Multi-Spectral Sentinel-1/2 \\ Imagery for Deep Learning and Data Fusion\end{tabular} &
  256 x 256 &
  541,986 &
  10 &
  \begin{tabular}[c]{@{}c@{}}Sentinel-1,\\ Sentinel-2,\\ MODIS Land\\ Cover\end{tabular} &
  33 &
  Globally distributed &
  SAR/Multispectral &
  \begin{tabular}[c]{@{}c@{}}Land Cover Classification, \\ Change Detection,\end{tabular} \\
Jun, 2019 &
  BigEarthNet \cite{Sumbul_2019_Bigearthnet} &
  \begin{tabular}[c]{@{}c@{}}BigEarthNet: A Large-Scale Benchmark \\ Archive For Remote Sensing \\ Image Understanding\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}20 x 20 \\ to 120 x 120\end{tabular} &
  590,326 &
  Various &
  Sentinel-2 &
  43 &
  Europe &
  Multispectral &
  \begin{tabular}[c]{@{}c@{}}Scene Classification, \\ Object Detection\end{tabular} \\
Jun, 2019 &
  SeCo \cite{SeCo} &
  \begin{tabular}[c]{@{}c@{}}Seasonal Contrast: Unsupervised Pre-Training \\ from Uncurated Remote Sensing Data\end{tabular} &
  264 x 264 &
  $\sim$1M &
  10 - 60 &
  Sentinel-2 &
  - &
  Global &
  Multispectral &
  \begin{tabular}[c]{@{}c@{}}Seasonal Change Detection, \\ Land Cover Classification \\ over Seasons\end{tabular} \\
Mar, 2021 &
  MillionAID \cite{Long2022ASP_millionaid, Long2021DiRS_millionaid}&
  Million-AID &
  110 - 31,672 &
  1,000,848 &
  Various &
  Google Earch &
  51 &
  Global &
  RGB &
  Scene Classification \\
Jul, 2021 &
  Levir-KR \cite{GeoKR} &
  \begin{tabular}[c]{@{}c@{}}Geographical Knowledge-driven \\ Representation Learning for \\ Remote Sensing Images\end{tabular} &
  - &
  1,431,950 &
  Various &
  \begin{tabular}[c]{@{}c@{}}Gaofen1, \\ Gaofen-2, \\ Gaofen-6\end{tabular} &
  8 &
  Global &
  Multispectral &
  \begin{tabular}[c]{@{}c@{}}Change Detection, \\ Scene Classification\end{tabular} \\
% Aug, 2021 &
%   SoundingEarth \cite{heidler2021SoundingEarth} &
%   - &
%   1024 x 1024 &
%   50,545 &
%   0.2 &
%   Google Earth &
%   - &
%   Global &
%   RGB - Audio &
%   - \\
Apr, 2022 &
  TOV-RS-Balanced \cite{tao2022tovoriginalvisionmodel} &
  \begin{tabular}[c]{@{}c@{}}TOV: The Original Vision Model for Optical \\ Remote Sensing Image Understanding via \\ Self-supervised Learning\end{tabular} &
  600 x 600  &
  500,000 &
  1 - 20 &
  Google Earth &
  31 &
  Global &
  RGB &
  \begin{tabular}[c]{@{}c@{}}Scene Classification, \\ Object Detection, \\ Semantic Segmentation\end{tabular} \\
Jul, 2022 &
  SeasoNet \cite{koßmann2022seasonetseasonalsceneclassification}&
  \begin{tabular}[c]{@{}c@{}}SeasoNet: A Seasonal Scene Classification, \\ Segmentation and Retrieval dataset\\ for satellite Imagery over Germany\end{tabular} &
  up to 120 x 120 &
  1,759,830 &
  10 - 60 &
  Sentinel-2 &
  33 &
  Germany &
  Multispectral &
  \begin{tabular}[c]{@{}c@{}}Scene Classification,\\ Scene Segmentation\end{tabular} \\
Nov, 2022 &
  SSL4EO-S12 \cite{wang2023ssl4eos12largescalemultimodalmultitemporal} &
  \begin{tabular}[c]{@{}c@{}}SSL4EO-S12: A Large-Scale Multi-Modal, \\ Multi-Temporal Dataset for Self-Supervised \\ Learning in Earth Observation\end{tabular} &
  264 x 264 &
  3,012,948 &
  10 - 60 &
  \begin{tabular}[c]{@{}c@{}}Sentinel-1, \\ Sentinel-2\end{tabular} &
  - &
  Global &
  SAR/Multispectral &
  \begin{tabular}[c]{@{}c@{}}Scene Classification, \\ Object Detection\end{tabular}
\end{tabular}%
}
\end{adjustbox}
\caption{This table summarizes a set of most commonly used pre-trained datasets for remote sensing.}
\label{tab:pre-train_datasets}
\end{sidewaystable*}




==> tables/Used_segmentation.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}
\begin{sidewaystable*}
\centering
\begin{adjustbox}{width=\textwidth}{!}{%
\begin{tabular}{cc
>{\columncolor[HTML]{FFF2CC}}c ccccccc}
\cellcolor[HTML]{D9E7FD}\textbf{Year-Month} &
  \cellcolor[HTML]{D9E7FD}\textbf{Architecture} &
  \cellcolor[HTML]{D9EAD3}\textbf{Model Name} &
  \cellcolor[HTML]{D9E7FD}\textbf{Pre-training Dataset} &
  \cellcolor[HTML]{D9E7FD}\textbf{Resolution (m)} &
  \cellcolor[HTML]{D9E7FD}\textbf{Geographic Coverage} &
  \cellcolor[HTML]{D9E7FD}\textbf{Visual Encoder} &
  \cellcolor[HTML]{D9E7FD}\textbf{Pretrain methods} &
  \cellcolor[HTML]{D9E7FD}\textbf{\# of Params} \\
2021 Oct &
  ResNet-50 &
  GeoKR \cite{GeoKR} &
  Levir-KR \cite{GeoKR}&
  0.8 to 16 &
  Global &
  ResNet-50/VGG16 &
  \begin{tabular}[c]{@{}c@{}}Geographical Knowledge\\ Supervision\end{tabular} &
  23.5M/138M \\
2021 Oct &
  ResNet-50 &
  SeCo \cite{SeCo}&
  Sentinel-2 Imagery &
  10, 20, 60 &
  \begin{tabular}[c]{@{}c@{}}200k Locations \\ Worldwide\end{tabular} &
  ResNet-50 &
  CL &
  23.5M \\
2022 Jun &
  ViT-S/8 &
  DINO-MM \cite{DINO-MM}&
  BigEarthNet - MM &
  10 &
  Global &
  ViT-S/8 &
  SSL &
  22M \\
2023 Jan &
  \begin{tabular}[c]{@{}c@{}}MAE-based \\ Framework\end{tabular} &
  SatMAE \cite{SatMAE} &
  fMoW Sentinal-2 &
  10, 20, 60 &
  Global &
  ViT-Large &
  MAE &
  307M \\
2022 Sep &
  BYOL &
  RS-BYOL \cite{RS-BYOL}&
  Sen12MS \cite{schmitt2019sen12mscurateddataset}&
  10 to 20 &
  Global &
  ResNet-50 &
  SSL &
  23.5M \\
2022 Aug &
  ResNet-50 &
  GeCO \cite{GeCo}&
  Levir-KR \cite{GeoKR}&
  0.8 to 16 &
  Global &
  ResNet-50 &
  SSL &
  23.5M \\
2022 Jul &
  ViT/Swin Transformer &
  RingMo \cite{RingMo}&
  2 million RS images &
  0.3 to 30 &
  6 Continents &
  ViT/Swin Transformer &
  MIM &
  - \\
2022 Nov &
  ViT &
  RVSA \cite{RVSA}&
  MillionAID \cite{Long2022ASP_millionaid, Long2021DiRS_millionaid}&
  0.5 to 153 &
  Global &
  ViT-B/ViTAE-B &
  MAE &
  100M \\
2021 Dec &
  ResNet-34 &
  MATTER \cite{MATTER}&
  Sentinel-2 Imagery &
  -  &
  \begin{tabular}[c]{@{}c@{}}Rural and Remote Regions\\ with Little Changes\end{tabular} &
  ResNet-34 &
  SSL &
  21.3M \\
2022 Nov &
  ViT-B &
  CSPT \cite{CSPT}&
  ImageNet-1K &
  - &
  Global &
  ViT-B &
  SSL &
  86M \\
2022 Jun &
  Swin Transformer &
  Scheibenreif, et al. \cite{Scheibenreif_2022_CVPR}&
  SEN12MS &
  10 &
  Global &
  Swim Transformer &
  CL &
  - \\
2023 Apr &
  TOV &
  TOV \cite{TOV}&
  \begin{tabular}[c]{@{}c@{}}TOV-NI,\\ TOV-RS\end{tabular} &
  - &
  Global &
  ViT &
  SSL &
  - \\
2023 Apr &
  \begin{tabular}[c]{@{}c@{}}Teacher-student\\ Self-distillation\end{tabular} &
  CMID \cite{CMID}&
  MillionAID \cite{Long2022ASP_millionaid, Long2021DiRS_millionaid}&
  Varied &
  Global &
  ResNet-50/Swin-B &
  SSL &
  25.6M/87.8M \\
2023 Jun &
  ResNet-18 &
  IaI-SimCLR \cite{IaI-SimCLR}&
  SEN12MS &
  - &
  Global &
  ResNet-18 &
  CL &
  11.7M \\
2023 Jun &
  CACo &
  CACo \cite{CACo}&
  Sentinel-2 Imagery &
  10 &
  Global &
  ResNet-18/50 &
  SSL &
  11.7M/23.5M \\
2023 Aug &
  Swim Transformer &
  SatLasPretrain \cite{SatlasPretrain} &
  SatLasPretrain &
  1, 10 &
  All Continents except Antarctica &
  Swim Transformer &
  Pretrained on Dataset &
  - \\
2023 Aug &
  Teacher-Student &
  GFM \cite{GFM}&
  GeoPile &
  - &
  Global &
  Swim Transformer &
  Continual Pretraining &
  - \\
2023 Sep &
  ViT &
  Scale-MAE \cite{Scale-MAE}&
  fMoW \cite{fmow2018}&
  - &
  Global &
  ViT-Large &
  MAE &
  322.9M \\
2024 Apr &
  DINO &
  DINO-MC \cite{DINO-MC}&
  SeCo-100K \cite{SeCo}&
  10 to 60 &
  Global &
  \begin{tabular}[c]{@{}c@{}}ViT,\\ Swim Transformer,\\ ResNet,\\ WRN\end{tabular} &
  SSL &
  - \\
2023 Nov &
  Multimodal Encoder &
  CROMA \cite{CROMA}&
  SSL4EO \cite{wang2023ssl4eos12largescalemultimodalmultitemporal}&
  10 &
  \begin{tabular}[c]{@{}c@{}}Areas Surrounding \\ Human Settlements\end{tabular} &
  ViT-B &
  CL, MAE &
  86M \\
2024 Jan &
  ViT-B &
  Cross-Scale MAE \cite{Cross-Scale-MAE}&
  fMoW \cite{fmow2018}&
  - &
  Global &
  ViT-B &
  MAE &
  86M \\
2023 Sep &
  Multimodel SSL &
  DeCUR \cite{DeCUR}&
  \begin{tabular}[c]{@{}c@{}}SSL4EO-S12, \\ RGB-DEM/depth\end{tabular} &
  Varied &
  Global &
  ResNet-50 &
  SSL &
  23.5M \\
2024 May &
  ViT &
  CtxMIM \cite{CtxMIM}&
  WorldView-3 Imagery &
  Varied &
  Asia &
  Swim-B &
  MIM &
  88M \\
2023 Oct &
  ViT &
  FG-MAE \cite{FG-MAE}&
  SSL4EO-S12 \cite{wang2023ssl4eos12largescalemultimodalmultitemporal}&
  10 &
  Global &
  ViT &
  MAE &
  - \\
2023 Oct &
  ViT &
  Prithvi \cite{Prithvi}&
  Harmonized Landsat Sentinel 2 &
  30 &
  Contiguous U.S. &
  ViT &
  MAE &
  100M \\
2023 Sep &
  CNN-Transformer &
  RingMo-lite \cite{RingMo-lite}&
  AID \cite{Xia_2017}&
  0.3 to 30 &
  Global &
  Swim Transformer + CNN &
  FD-MIM &
  60\% less than RingMo \\
2023 Oct &
  MSFE+MMFH &
  Feng et al. \cite{Feng2023}&
  Multi-modal Dataset &
  Varied &
  Global &
  Transformer &
  SSL &
  - \\
2024 Jan &
  ViT &
  USat \cite{USat}&
  Satlas &
  Varied &
  Global &
  ViT &
  MAE &
  - \\
2024 Mar &
  ViT &
  FoMo-Bench \cite{FoMo-Bench}&
  Multiple &
  Varied &
  Global &
  ViT &
  MAE &
  101M/110M \\
2024 Jan &
  Unet+Transformer &
  U-BARN \cite{U-BARN}&
  Sentinel-2 Imagery &
  Varied &
  France &
  Unet+Transformer &
  SSL &
  - \\
2024 Jan &
  \begin{tabular}[c]{@{}c@{}}Teacher-Student \\ Network\end{tabular} &
  GeRSP \cite{GeRSP}&
  ImageNet\cite{imageNet}, MillionAID\cite{Long2022ASP_millionaid, Long2021DiRS_millionaid} &
  0.5 to 153 &
  Global &
  ResNet-50 &
  SSL, SL &
  - \\
2024 Jan &
  Dual-Branch &
  SwiMDiff \cite{SwiMDiff}&
  Sen12MS \cite{schmitt2019sen12mscurateddataset} &
  Varied &
  Global &
  ResNet-18 &
  SSL &
  11.7M \\
2024 May &
  OFA-Net &
  OFA-Net \cite{OFA-Net}&
  Multi-modal Dataset &
  Varied &
  Global &
  ViT &
  MIM &
  - \\
2024 Feb &
  3D GPT &
  SpectralGPT \cite{SpectralGPT}&
  Sentinel-2 Imagery &
  Varied &
  Global &
  ViT &
  MAE &
  100M/300M/600M \\
2024 May &
  HiViT &
  SARATR-X \cite{SARATR-X}&
  SAR Datasets &
  0.1 to 3 &
  Global &
  HiViT &
  MIM &
  66M \\
2024 Mar &
  SatMAE &
  SatMAE++ \cite{SatMAE++}&
  fMoW \cite{fmow2018} &
  Varied &
  Global &
  ViT-Large &
  \begin{tabular}[c]{@{}c@{}}Multi-Scale\\ Pre-training\end{tabular} &
  - \\
2024 Apr &
  Swim Transformer &
  msGFM \cite{msGFM}&
  GeoPile-2 &
  0.1 to 153 &
  Global &
  Swim Transformer &
  MIM &
  89M \\
2024 Mar &
  \begin{tabular}[c]{@{}c@{}}Factorized Multi-Modal\\ Spatiotemporal Encoder\end{tabular} &
  SkySense \cite{SkySense}&
  Multiple &
  Varied &
  Global &
  Multiple &
  CL &
  2.06B \\
2024 May &
  \begin{tabular}[c]{@{}c@{}}Shared Encoder\\ Task-Specific Decoders\end{tabular} &
  MTP \cite{MTP}&
  SAMRS &
  Varied &
  Global &
  \begin{tabular}[c]{@{}c@{}}RVSA,\\ InternImage\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Multi-Task \\ Pretraining\end{tabular} &
  over 300M \\
2024 Jun &
  Dynamic OFA &
  DOFA \cite{DOFA}&
  Multiple &
  Varied &
  Global &
  ViT &
  MIM &
  - \\
2024 Mar &
  Multi-Modules &
  UPetu \cite{UPetu}&
  GeoSense &
  - &
  Global &
  ConvNeXt-B &
  SSL &
  0.65M \\
2024 May &
  MP-MAE &
  MMEarth \cite{MMEarth}&
  \begin{tabular}[c]{@{}c@{}}Multi-modal,\\ Geospatial Data\end{tabular} &
  - &
  Global &
  ConvNeXt V2 &
  MP-MAE &
  3.7M to 650M

\end{tabular}%
}
\end{adjustbox}
\caption{Summary of foundation models for semantic segmentation in remote sensing, detailing architecture, pre-training datasets, resolution, geographic coverage, visual encoders, pretraining methods, and number of parameters.}
\label{tab:scene_segmentation}
\end{sidewaystable*}

==> tables/combined_cv_models_table.tex <==


\begin{document}

\begin{longtable}{|c|c|c|c|c|c|c|c|}
\hline
\cellcolor[HTML]{D9E7FD}\textbf{Architecture} &
\cellcolor[HTML]{D9E7FD}\textbf{Model Name} &
\cellcolor[HTML]{D9E7FD}\textbf{Pre-training Dataset} &
\cellcolor[HTML]{D9E7FD}\textbf{Resolution (m)} &
\cellcolor[HTML]{D9E7FD}\textbf{Geographic Coverage} &
\cellcolor[HTML]{D9E7FD}\textbf{Downstream Tasks} &
\cellcolor[HTML]{D9E7FD}\textbf{Pre-train Methods} &
\cellcolor[HTML]{D9E7FD}\textbf{\# of Params} \\
\hline
\endfirsthead

\hline
\cellcolor[HTML]{D9E7FD}\textbf{Architecture} &
\cellcolor[HTML]{D9E7FD}\textbf{Model Name} &
\cellcolor[HTML]{D9E7FD}\textbf{Pre-training Dataset} &
\cellcolor[HTML]{D9E7FD}\textbf{Resolution (m)} &
\cellcolor[HTML]{D9E7FD}\textbf{Geographic Coverage} &
\cellcolor[HTML]{D9E7FD}\textbf{Downstream Tasks} &
\cellcolor[HTML]{D9E7FD}\textbf{Pre-train Methods} &
\cellcolor[HTML]{D9E7FD}\textbf{\# of Params} \\
\hline
\endhead

\hline
\endfoot

[c]{@{}c@{}}Scene Classification, \\ Semantic Segmentation
[c]{@{}c@{}}Scene Classification, \\ Semantic Segmentation
\hline
\end{longtable}

\caption{Overview of recent foundation models in remote sensing, categorized by architecture, model name, pre-training dataset, resolution, geographic coverage, CV-applications, visual encoder, pre-training methods, and the number of parameters. Abbreviations for pre-training methods: SSL refers to Self-Supervised Learning, CL stands for Contrastive Learning, MIM is Masked Image Modeling, MAE is Masked Autoencoders, and FD-MIM is Feature-Distilled Masked Image Modeling. *Resolution in degrees indicates global-scale coverage, where each pixel spans approximately 1.40625 degrees in latitude and longitude.}

\label{tab:combined-cv-models}
\end{document}


==> texts/datasets.tex <==
\section{Datasets}
Datasets play a crucial role in remote sensing, providing the foundation for training and evaluating models. High-quality datasets enable models to learn accurate representations of the Earth's surface, improving their performance on various remote sensing tasks. In this section, we provide an overview of commonly used datasets in table \ref{tab:pre-train_datasets} for remote sensing, discussing their characteristics, applications, and relevance to foundation models. These datasets, with their varying resolutions, categories, and geographic coverage, provide a rich resource for advancing remote sensing research and applications. They facilitate the development of robust models capable of addressing diverse challenges in understanding and interpreting Earth's surface through remote sensing technologies.

\hl{Datasets used in remote sensing vary significantly in size, from hundreds of thousands of samples, as in RSD46-WHU }\cite{Long2017, Xiao2017}\hl{, to over a million, as seen in MillionAID }\cite{Long2022ASP_millionaid, Long2021DiRS_millionaid}\hl{Generally, larger datasets contribute to model generalization by encompassing diverse geographic areas, seasonal variations, and environmental conditions. Dataset resolutions also range from high (sub-meter), suitable for tasks requiring detailed spatial analysis, to moderate (10-60 meters), as with SEN12MS }\cite{schmitt2019sen12mscurateddataset}\hl{ and SSL4EO-S12 } \cite{wang2023ssl4eos12largescalemultimodalmultitemporal}\hl{, which support broader pattern recognition applications.}

\footnotetext{Object detection and Segmentation © MAXAR 2024, provided through the NextView License Agreement.}

\hl{These datasets leverage various sensor types, including RGB, multispectral, hyperspectral, and synthetic aperture radar (SAR). For instance, SEN12MS} \cite{schmitt2019sen12mscurateddataset}\hl{ integrates both SAR and multispectral imagery, enabling models to learn from distinct data modalities. This diversity in sensor types is critical for robust model development, as each sensor type captures unique surface characteristics, supporting tasks that benefit from cross-modal information.

Foundation models, in particular, benefit from such large-scale, multimodal datasets, which support self-supervised and supervised training approaches across tasks such as scene classification, segmentation, and object detection. For further insight, the appendix includes detailed descriptions of each dataset’s structure, unique characteristics, and application roles, enhancing the understanding of their impact on remote sensing advancements.}




% The RSD46-WHU \cite{Long2017, Xiao2017} dataset, introduced in 2017, is sourced from Google Earth and Tianditu. It contains 117,000 images with a patch size of 256 pixels and spatial resolutions ranging from 0.5 to 2 meters per pixel. Covering 46 categories globally, this dataset is primarily used for scene classification. Similarly, the Functional Map of the World (fMoW) \cite{fmow2018}, released in April 2018, comprises over 1 million images from Digital Globe. Spanning 63 categories across 207 countries, it includes multispectral images used for both scene classification and object detection.

% In May 2019, the DOTA \cite{xia2019dotalargescaledatasetobject} dataset was proposed, known for its large-scale aerial image object detection capabilities. It includes 11,268 images of various resolutions from Google Earth, GF-2 Satellite, and aerial sources, covering 18 categories globally. Another significant dataset, SEN12MS \cite{schmitt2019sen12mscurateddataset}, released in June 2019, contains 541,986 images from Sentinel-1, Sentinel-2, and MODIS Land Cover. With a patch size of 256x256 pixels, it supports land cover classification and change detection tasks.

% BigEarthNet \cite{Sumbul_2019_Bigearthnet}, also from June 2019, consists of 590,326 images with varying sizes from 20x20 to 120x120 pixels, sourced from Sentinel-2. It covers 43 categories across Europe and is used for scene classification and object detection. The SeCo \cite{SeCo} dataset, another June 2019 release, contains approximately 1 million images with a resolution of 2.65x2.65km from Sentinel-2. It is designed for seasonal change detection and land cover classification over seasons.

% The MillionAID dataset \cite{Long2021DiRS_millionaid, Long2022ASP_millionaid}, introduced in March 2021, includes over 1 million images of various sizes from Google Earth. Covering 51 categories globally, it is used for scene classification. Levir-KR, released in July 2021, contains 1,431,950 images from Gaofen-1, Gaofen-2, and Gaofen-6 satellites, supporting change detection and scene classification applications.

% SoundingEarth \cite{heidler2021SoundingEarth}, introduced in August 2021, comprises 50,545 images of 1024-pixel size from Google Earth, combining RGB and audio data for remote sensing. The TOV-RS-Balanced dataset \cite{tao2022tovoriginalvisionmodel} from April 2022 includes 500,000 images with a 600-pixel size from Google Earth, covering 31 categories globally, and is used for scene classification, object detection, and semantic segmentation.

% \footnotetext{RGB Image and Segmentation © MAXAR 2024, provided through the NextView License Agreement.}

% SeasoNet \cite{koßmann2022seasonetseasonalsceneclassification}, released in July 2022, features 1,759,830 images from Sentinel-2 with patch size from 20 to 120 pixels, supporting seasonal scene classification, segmentation, and retrieval over Germany. Lastly, the SSL4EO-S12 dataset \cite{wang2023ssl4eos12largescalemultimodalmultitemporal} from November 2022 contains over 3 million images from Sentinel-1 and Sentinel-2, with patch size of 264x264 pixels. It is used for scene classification and object detection.

% These datasets, with their varying resolutions, categories, and geographic coverage, provide a rich resource for advancing remote sensing research and applications. They facilitate the development of robust models capable of addressing diverse challenges in understanding and interpreting Earth's surface through remote sensing technologies.

% \input{tables/Used_pre-train_datasets}




==> texts/models.tex <==
%% the format of the tables need to change later, something is wrong
\section{Foundation Models for Remote Sensing}
\label{sec:models}
In this section, we \hl{present two parallel types of categorization to organize the use of foundation models} in remote sensing. \hl{The first categorization focuses on computer vision tasks, such as scene classification, semantic segmentation, and object detection, which represent general techniques for analyzing image data. These tasks serve as the foundation for most remote sensing applications, as they provide the underlying technical framework for processing and interpreting imagery. The second categorization is based on domain-specific applications, such as environmental monitoring} \cite{Himeur2022}, \hl{urban planning}\cite{Jha2021}\hl{, disaster management}\cite{Abid2021}\hl{, and so on. These applications often rely on one or more of the core computer vision tasks but are tailored to address particular real-world challenges within specific domains. For example, deforestation tracking typically involves semantic segmentation to map forest cover, while urban planning may utilize object detection to identify buildings or infrastructure in satellite imagery. This dual categorization allows for a clearer understanding of how foundation models apply both general computer vision techniques and specialized domain knowledge in the field of remote sensing.}

\footnotetext{RGB Image and Segmentation © MAXAR 2024, provided through the NextView License Agreement.}

\subsection{Computer Vision Tasks}

Computer vision tasks involve the automatic analysis and interpretation of imagery to extract meaningful information.\hl{In the context of remote sensing, the primary tasks include scene classification, semantic segmentation, object detection, change detection, and instance segmentation.} Each of these tasks requires different model architectures and training methodologies to achieve optimal performance. \hl{Pretraining methods are used to initialize models with unlabeled data, enabling them to learn useful representations. Self-Supervised Learning (SSL) encompasses a variety of techniques, including Contrastive Learning (CL), where models learn by comparing similar and dissimilar samples. Masked Image Modeling (MIM) involves predicting masked parts of an image, while Masked Autoencoding (MAE) is a specific type of MIM that uses an encoder-decoder framework to reconstruct the masked regions.} The following sections provide an overview of various models used for these tasks, along with their specific applications and performance metrics. Table \ref{tab:CV_task} summarizes those downstream tasks tested by each vision models.

    % \input{tables/Use_CV_tasks}

    %-----------------------------------
    \subsubsection{\textbf{Scene Classification}}
Scene classification in remote sensing involves categorizing images or parts of images into predefined classes, such as urban, forest, water bodies, and agricultural areas. This task is crucial for land use and land cover mapping, environmental monitoring, and urban planning. Accurate scene classification enables better resource management and policy-making by providing detailed and up-to-date information about land cover and land use patterns. In table \ref{tab:cv-task1} and \ref{tab:cv-task2}, we provide an overview of various foundation models used for scene classification in remote sensing.
         
        % \input{tables/Used_Scene_Classification}
        % \FloatBarrier
    %-----------------------------------   
    \subsubsection{\textbf{Semantic Segmentation}} 
Semantic segmentation is a crucial task in the field remote sensing that involves classifying each pixel in an image into a predefined category. This task is crucial for creating detailed maps that show the distribution of different land cover types, such as forests, water bodies, urban areas, and agricultural fields. The high-resolution, pixel-level information provided by semantic segmentation is essential for applications in environmental monitoring, urban planning, disaster management, and precision agriculture. In table \ref{tab:cv-task1} and \ref{tab:cv-task2}, we provide an overview of various foundation models used for semantic segmentation in remote sensing. 

        % \input{tables/Used_segmentation}
        % \FloatBarrier
    %-----------------------------------          
    \subsubsection{\textbf{Object Detection}} 
Object detection is a critical task in remote sensing that involves identifying and locating objects within an image. Unlike scene classification and semantic segmentation, which focus on classifying entire images or individual pixels, object detection aims to recognize specific objects, such as vehicles, buildings, ships, and other structures, and determine their positions within the image. This task is essential for applications in urban planning, environmental monitoring, disaster response, and security. Table \ref{tab:cv-task1} and \ref{tab:cv-task2} summarize all foundation models that can be used for remote sensing object detection tasks. 

        % \input{tables/Used_object_detection}
        % \FloatBarrier
    %-----------------------------------
    \subsubsection{\textbf{Change Detection}} 
Change detection in remote sensing involves identifying and analyzing changes in the Earth's surface over time by comparing images taken at different times. This task is vital for monitoring environmental changes, urban expansion, deforestation, natural disasters, and other dynamic phenomena. By detecting changes accurately, change detection provides crucial insights for environmental management, urban planning, disaster response, and climate change studies. Foundation models that can accomplish change detection tasks are listed in table \ref{tab:cv-task1} and \ref{tab:cv-task2}. 
    % \input{tables/Used_Scene_Classification}
    % \FloatBarrier

    % \input{tables/Used_segmentation}
    % \FloatBarrier

    % \input{tables/Used_object_detection}
    % \FloatBarrier
    
    % \input{tables/Used_change_detection}
    % \FloatBarrier

    \input{tables/cv_model1}
    \input{tables/cv_model2}
    % \input{tables/cv_model}

%%%%%%%%%%%%%%%%% Challenges for CV tasks         
    \subsubsection{\textbf{Unique Challenges for Applied Computer Vision Task in Remote Sensing}}
Applying computer vision (CV) techniques to remote sensing presents several unique challenges distinct from other fields. In traditional computer vision, \hl{models} often focus on detecting and classifying discrete objects, such as animals or vehicles, with the rest of the image considered background. However, in remote sensing, the concept of "background" is no longer existed: every pixel contains valuable information about the Earth's surface. This necessitates CV methods that can analyze entire images comprehensively rather than isolating specific objects. This idea is highlighted by Li et al. in their research that remote sensing images classification requires advanced techniques that can handle the complexity and variability inherent in pixel-wise data\cite{Li2018survey}.

Another significant challenge is the sensor-specific nature of remote sensing data. Unlike the standardized pixel values in typical CV tasks, remote sensing images are captured by various sensors (e.g., optical, radar) that measure physically meaningful quantities. These measurements depend on the sensor technology, requiring CV algorithms to account for differences such as point spread function and spectral response function of the sensors. As discussed by Roy et al. \cite{roy2017satellite}, advancements in sensor technology, including the development of high-resolution optical and radar systems, have significantly impacted the way remote sensing data is processed and analyzed.

Moreover, remote sensing tasks involve diverse and complex data, varying in resolution, spectral characteristics, and temporal aspects. This diversity demands CV methods adaptable to different imaging conditions, such as varying times of day, seasons, and weather, which significantly affect the appearance of geographic areas. Traditional CV techniques, typically developed for more uniform datasets, often struggle with such variability. For example, in crop monitoring, as discussed by Han et al. \cite{Han2024}, fluctuations in weather conditions and variations in sensor data introduce significant variability, making it challenging to accurately assess crop health and yield using remote sensing techniques.

To address these challenges, integrating deep learning techniques from CV with domain-specific knowledge in remote sensing is essential. This approach can enhance the robustness and accuracy of methods tailored to the complexities of remote sensing data. In the following section, we will discuss these different domain-specific tasks in details. 

%%%%%%%% Domain-specific
\subsection{Domain-Specific Tasks}
Domain-specific tasks in remote sensing refer to applications that address particular real-world challenges by leveraging the capabilities of foundation models. These tasks include environmental monitoring, archaeology, agriculture, urban planning and development, and disaster management. To highlight the versatility of foundation models in remote sensing, we present 
\hl{table} \ref{tab:cv-domain} that categorizes models based on their applicability to various domain-specific tasks, as well as computer vision tasks. This figure serves as a quick reference for researchers to identify suitable models for their specific needs.

% \begin{figure*}
%     \centering
%     \includegraphics[width=\textwidth]{figures/fig6_domain-CV.pdf}
%     \caption{This diagram illustrates various domain-specific tasks in computer vision and their connections. Key areas include Environmental Monitoring, Agriculture and Forestry, Urban Planning and Development, Disaster Management, and Archaeology. Each domain comprises specific tasks such as change detection and object Detection. The relationships between these tasks and their application domains are depicted through connecting arrows, emphasizing the interconnected nature of computer vision applications across different fields.}
%     \label{fig:domain-cv-tasks}
% \end{figure*}

\input{tables/CV_domain}
% \input{tables/model_test}

        
    \subsubsection{\textbf{Environmental Monitoring}}
\hl{According to Himeur et al. (2022), environmental monitoring utilizes remote sensing models to observe and track environmental changes, including deforestation, desertification, and pollution. These models play a crucial role in analyzing the effects of human activities and natural phenomena on the environment }\cite{Himeur2022}.

    \subsubsection{\textbf{Agriculture}}
\hl{In agriculture, remote sensing models are used to monitor crop health, estimate yields, and manage agricultural practices. According to Kamilaris et al. (2018), these models help optimize resource use and improve agricultural productivity} \cite{Kamilaris2018}. 

    \subsubsection{\textbf{Archaeology}}
\hl{In archaeology, remote sensing models have been used to identify and analyze archaeological features and sites. According to Argyrou et al. (2022), these models help detect features such as ruins, artifacts, and ancient structures from satellite imagery, leveraging technologies like Convolutional Neural Networks (CNNs) and Vision Transformers (ViTs) to process high-resolution images and capture fine details }\cite{Argyrou2022}. \hl{Mantovan et al. (2020) also highlight the effectiveness of AI models, particularly CNNs, in locating challenging terrestrial archaeological sites and processing multispectral data} \cite{Mantovan2020}.
            
            
    \subsubsection{\textbf{Urban Planning and Development}}
\hl{In urban planning and development, remote sensing models are used to monitor and analyze urban expansion, infrastructure development, and land use changes. According to Jha et al. (2021), these models play a critical role in managing urban growth, planning new developments, and assessing the impact of urbanization by providing essential data for smart city planning and sustainable development }\cite{Jha2021}.

            
    \subsubsection{\textbf{Disaster Management}}
\hl{Remote sensing models play a crucial role in disaster management by providing timely information on affected areas. According to Abid et al. (2021), these models are used to detect and assess damage from natural disasters like earthquakes, hurricanes, and floods, enabling rapid response and recovery efforts} \cite{Abid2021}.


        % \input{tables/domain_tasks}
